What is Local Optimality in Nonconvex-Nonconcave Minimax Optimization?

Minimax optimization has found extensive applications in modern machine learning, in settings such as generative adversarial networks (GANs), adversarial training and multi-agent reinforcement learning. As most of these applications involve continuous nonconvex-nonconcave formulations, a very basic question arises---"what is a proper definition of local optima?" Most previous work answers this question using classical notions of equilibria from simultaneous games, where the min-player and the max-player act simultaneously. In contrast, most applications in machine learning, including GANs and adversarial training, correspond to sequential games, where the order of which player acts first is crucial (since minimax is in general not equal to maximin due to the nonconvex-nonconcave nature of the problems). The main contribution of this paper is to propose a proper mathematical definition of local optimality for this sequential setting---local minimax, as well as to present its properties and existence results. Finally, we establish a strong connection to a basic local search algorithm---gradient descent ascent (GDA): under mild conditions, all stable limit points of GDA are exactly local minimax points up to some degenerate points.

==> optimality.tex <==
%!TEX root = main.tex

\section{What is the Right Objective?}\label{sec:obj}
\label{sec:optimality}

We have introduced three notions of optimality in minimax games:
global minimax points (Definition \ref{def:globalminimax}), pure strategy Nash equilibria (Definition \ref{def:pureNash}) and mixed strategy Nash equilibria (Definition \ref{def:mixedNash}). For convex-concave games, these three notions are essentially identical. However, for nonconvex-nonconcave games, they are all different in general. So, what is the right objective to pursue in this general setting?

\paragraph{Pure strategy Nash equilibrium} First, we note that pure strategy Nash equilibria may not exist in nonconvex-nonconcave settings.

\begin{proposition}
There exists a twice-differentiable function $f$, where \psnes (either local or global) do not exist.
\end{proposition}
\begin{proof}
Consider a two-dimensional function $f(x, y) = \sin (x+y)$. We have 
$\grad f(x, y) = (\cos(x+y), \cos(x+y))$.
Assuming $(x, y)$ is a local \psne, by Proposition \ref{prop:firstNash} it must also be a stationary point; that is, $x+y = (k+1/2)\pi$ for $k\in\Z$.
It is easy to verify, for odd $k$, $\phess_{xx} f (x, y)= \phess_{yy} f (x, y) = 1 > 0$; for even $k$, 
$\phess_{xx} f (x, y)= \phess_{yy} f (x, y) = -1 < 0$. By Proposition \ref{prop:secondNash}, none of the stationary points is a local \psne.
\end{proof}
Apart from the existence issue, the property that $\x^\star$ is optimal for $f(\cdot, \y^\star)$ is not meaningful in applications such as adversarial training, which translates to the property that the classifier needs to be optimal with respect to a fixed corruption.

\paragraph{Global minimax point} On the other hand, global \minimaxs, a simple but less mentioned notion of optimality, always exist.

\begin{proposition}\label{prop:minimaxexist}
Assume that function $f: \cX \times \cY \rightarrow \R$ is continuous, and assume that $\cX \subset \R^{d_1}$, $\cY \subset \R^{d_2}$ are compact. Then the global \minimax (Definition \ref{def:globalminimax}) of $f$ always exists.
\end{proposition}

% \begin{proof}
% For any fixed $\x$, since $\cY$ is compact, and $f(\x, \cdot)$ is continuous, by extreme value theorem, there exists $\y^\star_\x$ so that $f(\x, \y^\star_\x) = \sup_{\y\in \cY} f(\x, \y)$.
% Therefore, define $\phi(\x) \defeq \max_{\y\in \cY} f(\x, \y)$, it is not hard to verify that $\phi(\cdot)$ is also continuous. Since $\cX$ is also compact, by again extreme value theorem, there exists $\x^\star$ so that $\phi(\x^\star) = \inf_{\x \in \cX} \phi(\x)$. Then $(\x^\star, \y^\star_{\x^\star})$ is the global \minimax of $f$.
% % \cnote{Think about how to argue when max is at infinity.}
% \end{proof}

Proposition \ref{prop:minimaxexist} is a simple consequence of the extreme-value theorem. Compared to pure strategy Nash equilibria, the notion of global minimax is typically important in the setting where our goal is to find the best $\x^\star$ subject to adversarial perturbation of $\y$ rather than an $\x$ which is optimal for a fixed $\y^\star$. Indeed, both GANs and adversarial training actually fall in this category, where our primary goal is to find the best generator subject to an adversarial discriminator, and to find the best robust classifier subject to adversarial corruption.




==> pf_others.tex <==
%!TEX root = main.tex

\section{Proofs for Remaining Sections}

\PROPnoexist*

\begin{proof}
Consider a two-dimensional function $f(x, y) = \sin (x+y)$. We have 
$\grad f(x, y) = (\cos(x+y), \cos(x+y))$.
Assuming $(x, y)$ is a local \psne, by Proposition \ref{prop:firstNash} it must also be a stationary point; that is, $x+y = (k+1/2)\pi$ for $k\in\Z$.
It is easy to verify, for odd $k$, $\phess_{xx} f (x, y)= \phess_{yy} f (x, y) = 1 > 0$; for even $k$, 
$\phess_{xx} f (x, y)= \phess_{yy} f (x, y) = -1 < 0$. By Proposition \ref{prop:secondNash}, none of the stationary points is a local \psne.
\end{proof}

